On the Theoretical Equivalence of Several Trade-Off Curves Assessing Statistical Proximity

The recent advent of powerful generative models has triggered the renewed development of quantitative measures to assess the proximity of two probability distributions. As the scalar Frechet inception distance remains popular, several methods have explored computing entire curves, which reveal the trade-off between the fidelity and variability of the first distribution with respect to the second one. Several of such variants have been proposed independently and while intuitively similar, their relationship has not yet been made explicit. In an effort to make the emerging picture of generative evaluation more clear, we propose a unification of four curves known respectively as: the precision-recall (PR) curve, the Lorenz curve, the receiver operating characteristic (ROC) curve and a special case of R\'enyi divergence frontiers. In addition, we discuss possible links between PR / Lorenz curves with the derivation of domain adaptation bounds.

==> bound-simpler.tex <==
One of the most cited source exposing a useful upper bound for domain adaptation is \cite{ben2010theory}. The bound reads as follows:
\begin{equation*}
    \begin{split}
        \epsilon_T(h,f)\leq&\epsilon_S(h,f)+\gamma +\delta_{H\Delta H}(S,T)
    \end{split}
\end{equation*}
where, $\gamma:=\inf_{h'} \epsilon_S(h')+\epsilon_T(h')$ is the optimal combined error on source and target, and
$\delta_{H\Delta H}(\S,\T):=\sup_{h,h'\in H}\epsilon_T(h,h')-\epsilon_S(h,h')$ is called the $H\Delta H$-divergence, and accounts for how much two
hypotheses can deviate from one another and in a different way in the two domains.

As noted, in \cite{zhang2019bridging}, it is possible to improve their bound in several direction. 
In particular, they propose to adapt the bound by replace the $L^0$ error by differentiable loss like a margin loss. 
They also propose to improve the bounds by keeping it adaptive w.r.t the current hypothesis $h$.
Inpired by the derivations \cite{zhang2019bridging}, one can extract a refined version of the bound of \cite{ben2010theory}, as follows:

\begin{proposition}
\begin{equation}
    \begin{split}
        \epsilon_T(h,f)\leq&\epsilon_S(h,f)+\gamma+\delta(h,\S,\T)
    \end{split}
\end{equation}
where, $\gamma:=\inf_{h'} \epsilon_S(h')+\epsilon_T(h')$ is the optimal combined error on source and target, and
$\delta(h,\S,\T):=\sup_{h'}\epsilon_T(h,h')-\epsilon_S(h,h')$ is a kind of adaptive divergence, that accounts for 
how differently on $S$ and $T$ another hypothesis $h'$ can deviate from our current hypothesis $h$.
\end{proposition}
\begin{proof}
The proof is given mainly to highlight its use of the triangle identity $\epsilon_D(h,g)\leq \epsilon_D(h,f)+\epsilon_D(f,g)$ which 
is a pretty loose inequality.
\begin{equation*}
    \begin{split}
        \epsilon_T(h,f)\leq& \epsilon_T(h',f) +\underbrace{\epsilon_T(h,h')}_{=\epsilon_S(h,h')+\epsilon_T(h,h')-\epsilon_S(h,h')}\\
        \leq& \epsilon_T(h',f) + \underbrace{\epsilon_S(h,h')}_{\leq\epsilon_S(h,f)+\epsilon_S(h',f)} +\delta(h,\S,\T)\\
        \leq& \epsilon_S(h,f)+ \epsilon_S(h',f)+\epsilon_T(h',f) +\delta(h,\S,\T)
    \end{split}
\end{equation*}
This inequality being true for any arbitrary choice of $h'$, one can take the infimum of the right hand side w.r.t $h'$, which is the desired bound.
\end{proof}
\begin{remark}
The proof relies twice on the use of the triangle inequality, leading to a potential overestimate by a factor $3$. Indeed, if the best hypothesis is the same in the two domains, then $\gamma=2\inf_{h'}\epsilon_s(h',f)$.  And $h$ is approximately equal to this common best hypothesis, then the bound is at least 3 times as large as what is needed. 
\end{remark}

==> bound.tex <==
\section{Notations}
Let us denote $D_S$ and $D_T$ the joint distribution of input and labels respectively in the source and target domains. 
In general the inputs $x_S$ and $x_T$ may leave in different spaces $X_S$ and $X_T$. 
We also denote $Y$ the label space (which is common across the two domains).
For each domain $D\in\{S,T\}$ we denote $F_D$ the entire space of measurable functions from $X_D$ to $Y$. 

In what follows, we will denote $H_S$ the family of classifiers admissible in the source domain, and $H_T$ the family of classifiers in the target domains.
Because the source and target input spaces ($X_S$ and $X_T$) are potentially different, we also consider
$\Pi_{T\to S}$ (resp. $\Pi_{S\to T}$) a family of classifier adapters from $X_T$ to $X_S$ (resp. $X_S$ to $X_T$), that is to say :
$\forall \pi_S\in \Pi_{T\to S}, \forall h_T\in H_T, \pi_S.h_T$ is a classifier in the source domain (though possibly outside the family $H_S$).

We suppose that for each domain $D$ we have a labelling function $f_D\in F_D$, and we define for each classifier $h\in H_D$:
$$\epsilon_D(h,f_D):= Pr_D(h\neq f_D)$$

\section{An explanatory upper bound}

\begin{theorem} Let $h\in H_T$ and $\pi_S\in\Pi_{T\to S}$. Then
$$\epsilon_T(h,f_T)\leq \epsilon_S(\pi_S.h, f_S) + \delta_{h,\pi_S,H_S,\Pi_{S\to T}} + \lambda$$
where
$$\delta_{h,\pi_S,H_S,\Pi_{S\to T}}:=\sup_{\substack{h_S\in H_S\\ \pi_T\in \Pi_{S\to T}}} \epsilon_T(h,\pi_T.h_S) - \epsilon_S(\pi_S.h, h_S)$$
and
$$\lambda:=\lambda_S+\lambda_T = \inf_{\substack{h_S\in H_S\\ \pi_T\in \Pi_{S\to T}}} \epsilon_S(h_S, f_S)+\epsilon_T(\pi_T.h_S, f_T)$$
\end{theorem}

\begin{proof}
Let us choose an arbitrary pair $(h_S, \pi_T)\in H_S\times\Pi_{S\to T}$. One has (by using the triangular identity $\epsilon_D(f,f')\leq \epsilon_D(f,f'') + \epsilon_D(f'',f')$).
\begin{equation*}
    \begin{split}
        \epsilon_T(h,f_T)\leq& \epsilon_T(h,\pi_T.h_S) + \epsilon_T(\pi_T.h_S, f_T) \\
        &= \epsilon_T(\pi_T.h_S, f_T) + \epsilon_T(h,\pi_T.h_S) \\ 
        &= \epsilon_T(\pi_T.h_S, f_T) + \epsilon_S(h_S,\pi_S.h) + \epsilon_T(h,\pi_T.h_S) - \epsilon_S(h_S,\pi_S.h) \\
        \leq& \epsilon_T(\pi_T.h_S, f_T) + \underbrace{\epsilon_S(h_S,\pi_S.h)}_{\leq\epsilon_S(h_S,f_S)+\epsilon_S(\pi_S.h, f_S)} + \delta_{h,\pi_S,H_S,\Pi_{S\to T}}\\
        &= \epsilon_S(\pi_S.h, f_S) + \left( \epsilon_S(h_S,f_S) + \epsilon_T(\pi_T.h_S, f_T)\right) + \delta_{h,\pi_S,H_S,\Pi_{S\to T}}\\
    \end{split}
\end{equation*}
Since, $h_S$ and $\pi_T$ where fixed arbitrarily, one can consider a minimizing sequence such as $\epsilon_S(h_{S,n},f_S) + \epsilon_T(\pi_{T,n}.h_{S,n}, f_T) \xrightarrow[n\to\infty]{} \inf_{\substack{h_S\in H_S\\ \pi_T\in \Pi_{S\to T}}} \epsilon_S(h_S, f_S)+\epsilon_T(\pi_T.h_S, f_T) = \lambda$
\end{proof}


\begin{remark}
The previous bound is quite informative. It shows that a successful alignment is possible if :
\begin{enumerate}
    \item $\lambda$ is small, meaning that there exists a classifier $h_S\in H_S$ in the source domain and an adapter $\pi_T\in\Pi_{S\to T}$ onto the target domain, such that $h_S$ performs well in the source domain and $\pi_T.h_S$ performs well in the target domain.
    \item one optimizes $h$ and $\pi_S$ adversarially so as to minimize : 
    \begin{equation*}
    \begin{split}
    E(h,\pi_S):=&\epsilon_S(\pi_S.h, f_S) + \delta_{h,\pi_S,H_S,\Pi_{S\to T}} \\
    =& \epsilon_S(\pi_S.h, f_S) + \sup_{\substack{h_S\in H_S\\ \pi_T\in \Pi_{S\to T}}} \epsilon_T(h,\pi_T.h_S) - \epsilon_S(\pi_S.h, h_S)
    \end{split}
    \end{equation*}
\end{enumerate}
\end{remark}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{img/goodSituation.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

==> img/gaussianMixture.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Curve Lines [id:da11561889754006849] 
\draw [draw opacity=0][fill={rgb, 255:red, 218; green, 137; blue, 147 }  ,fill opacity=1 ][line width=2.25]    (133.97,196.89) .. controls (144.03,198.57) and (185.27,199.46) .. (191.68,216.13) .. controls (198.09,232.8) and (201.08,241.5) .. (203.22,252.04) .. controls (205.36,262.58) and (210.49,259.21) .. (203.22,258.45) .. controls (195.95,257.7) and (180.17,258.55) .. (162.18,258.45) .. controls (144.19,258.35) and (133.24,257.56) .. (133.33,258.45) ;
%Shape: Axis 2D [id:dp4272000883195448] 
\draw  (120.5,258.45) -- (248.75,258.45)(133.33,143.03) -- (133.33,271.28) (241.75,253.45) -- (248.75,258.45) -- (241.75,263.45) (128.33,150.03) -- (133.33,143.03) -- (138.33,150.03)  ;
%Shape: Right Angle [id:dp8764941173796803] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][dash pattern={on 6.75pt off 4.5pt}][line width=2.25]  (137.17,164.83) -- (226.95,164.83) -- (226.95,259) ;
%Shape: Axis 2D [id:dp7158274922933987] 
\draw  (274.4,258.45) -- (402.65,258.45)(287.23,143.03) -- (287.23,271.28) (395.65,253.45) -- (402.65,258.45) -- (395.65,263.45) (282.23,150.03) -- (287.23,143.03) -- (292.23,150.03)  ;
%Curve Lines [id:da491698761933099] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 218; green, 137; blue, 147 }  ,fill opacity=1 ][line width=2.25]    (377,168.68) .. controls (377.64,184.07) and (377.64,193.04) .. (377.64,212.28) .. controls (377.64,231.52) and (357.5,243.97) .. (351.99,249.48) .. controls (346.49,254.98) and (319.93,258.45) .. (287.23,258.45) ;
%Shape: Right Angle [id:dp45416924304215933] 
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][dash pattern={on 6.75pt off 4.5pt}][line width=2.25]  (377,168.68) -- (377,258.45) -- (287.23,258.45) ;
%Shape: Ellipse [id:dp2846094673872803] 
\draw  [draw opacity=0][fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (127.23,258.45) .. controls (127.23,255.09) and (129.96,252.36) .. (133.33,252.36) .. controls (136.69,252.36) and (139.42,255.09) .. (139.42,258.45) .. controls (139.42,261.82) and (136.69,264.54) .. (133.33,264.54) .. controls (129.96,264.54) and (127.23,261.82) .. (127.23,258.45) -- cycle ;
%Straight Lines [id:da8569644577698796] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=2.25]  [dash pattern={on 6.75pt off 4.5pt}]  (287.23,258.45) -- (380.85,164.83) ;
%Curve Lines [id:da5212349997924444] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (133.97,196.89) .. controls (144.03,198.57) and (185.27,199.46) .. (191.68,216.13) .. controls (198.09,232.8) and (203.22,245.63) .. (204.5,258.45) ;
%Image [id:dp5560744028403637] 
\draw (266.5,64.5) node  {\includegraphics[width=\linewidth,height=78.75pt]{img/mixture-PQ.png}};
%Straight Lines [id:da6312805275784865] 
\draw [color={rgb, 255:red, 0; green, 21; blue, 223 }  ,draw opacity=1 ][line width=1.5]    (396,24) -- (412.5,24) ;
%Straight Lines [id:da2666403555847445] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (396,44) -- (412.5,44) ;


% Text Node
\draw (142,130.74) node [anchor=north west][inner sep=0.75pt]    {$\alpha $};
% Text Node
\draw (235.62,226.93) node [anchor=north west][inner sep=0.75pt]    {$\beta $};
% Text Node
\draw (389.52,226.93) node [anchor=north west][inner sep=0.75pt]    {$t$};
% Text Node
\draw (298.16,130.74) node [anchor=north west][inner sep=0.75pt]    {$F( t)$};
% Text Node
\draw (143.35,267.79) node [anchor=north west][inner sep=0.75pt]   [align=left] {PR Curve };
% Text Node
\draw (312.53,268.11) node [anchor=north west][inner sep=0.75pt]   [align=left] {Lorenz curve};
% Text Node
\draw (416,31) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.82,0.01,0.11}{\T}$};
% Text Node
\draw (416,11) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0,0.08,0.87}{\S}$};


\end{tikzpicture}

==> img/gaussianMixture_old.tex <==

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=.75]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Curve Lines [id:da09266505411122883] 
\draw [draw opacity=0][fill={rgb, 255:red, 218; green, 137; blue, 147 }  ,fill opacity=1 ][line width=2.25]    (434.5,170) .. controls (432.27,170) and (415.12,250) .. (411.45,249.98) .. controls (407.77,249.96) and (378.88,249.72) .. (369.5,249) .. controls (360.12,248.28) and (353.5,251) .. (352.5,237) .. controls (351.5,223) and (350.5,201) .. (350.5,191) ;
%Curve Lines [id:da6936835813995819] 
\draw [draw opacity=0][fill={rgb, 255:red, 218; green, 137; blue, 147 }  ,fill opacity=1 ][line width=2.25]    (102.5,209) .. controls (110.35,210.31) and (142.5,211) .. (147.5,224) .. controls (152.5,237) and (154.83,243.78) .. (156.5,252) .. controls (158.17,260.22) and (162.17,257.59) .. (156.5,257) .. controls (150.83,256.41) and (138.53,257.08) .. (124.5,257) .. controls (110.47,256.92) and (101.93,256.31) .. (102,257) ;
%Shape: Axis 2D [id:dp41290010362368945] 
\draw  (92,257) -- (192,257)(102,167) -- (102,267) (185,252) -- (192,257) -- (185,262) (97,174) -- (102,167) -- (107,174)  ;
%Shape: Right Angle [id:dp040547899070892734] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][dash pattern={on 6.75pt off 4.5pt}][line width=2.25]  (105,184) -- (175,184) -- (175,254) ;
%Shape: Axis 2D [id:dp41060460298017376] 
\draw  (212,257) -- (312,257)(222,167) -- (222,267) (305,252) -- (312,257) -- (305,262) (217,174) -- (222,167) -- (227,174)  ;
%Curve Lines [id:da40304690956834666] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 218; green, 137; blue, 147 }  ,fill opacity=1 ][line width=2.25]    (292,187) .. controls (292.5,199) and (292.5,206) .. (292.5,221) .. controls (292.5,236) and (276.79,245.71) .. (272.5,250) .. controls (268.21,254.29) and (247.5,257) .. (222,257) ;
%Curve Lines [id:da5454362811287996] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (410.5,250) .. controls (402.5,250) and (382.5,250) .. (369.5,249) .. controls (356.5,248) and (353.5,251) .. (352.5,237) .. controls (351.5,223) and (350.5,201) .. (350.5,191) ;
%Shape: Axis 2D [id:dp3364553490381317] 
\draw  (332,257) -- (432,257)(342,167) -- (342,267) (425,252) -- (432,257) -- (425,262) (337,174) -- (342,167) -- (347,174)  ;
%Shape: Right Angle [id:dp1642242035367938] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][dash pattern={on 6.75pt off 4.5pt}][line width=2.25]  (412,257) -- (342,257) -- (342,187) ;
%Image [id:dp5560744028403637] 
\draw (266.5,64.5) node  {\includegraphics[width=250.5pt,height=78.75pt]{img/mixture-PQ.png}};
%Straight Lines [id:da6312805275784865] 
\draw [color={rgb, 255:red, 0; green, 21; blue, 223 }  ,draw opacity=1 ][line width=1.5]    (396,24) -- (412.5,24) ;
%Straight Lines [id:da2666403555847445] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (396,44) -- (412.5,44) ;

%Shape: Right Angle [id:dp4884488793677788] 
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][dash pattern={on 6.75pt off 4.5pt}][line width=2.25]  (292,187) -- (292,257) -- (222,257) ;
%Shape: Circle [id:dp054284216213610126] 
\draw  [draw opacity=0][fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (97.25,257) .. controls (97.25,254.38) and (99.38,252.25) .. (102,252.25) .. controls (104.62,252.25) and (106.75,254.38) .. (106.75,257) .. controls (106.75,259.62) and (104.62,261.75) .. (102,261.75) .. controls (99.38,261.75) and (97.25,259.62) .. (97.25,257) -- cycle ;
%Straight Lines [id:da5996222226091343] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=2.25]  [dash pattern={on 6.75pt off 4.5pt}]  (222,257) -- (295,184) ;
%Curve Lines [id:da054765458570643855] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (102.5,209) .. controls (110.35,210.31) and (142.5,211) .. (147.5,224) .. controls (152.5,237) and (156.5,247) .. (157.5,257) ;

% Text Node
\draw (109,158.4) node [anchor=north west][inner sep=0.75pt]    {$\alpha $};
% Text Node
\draw (182,233.4) node [anchor=north west][inner sep=0.75pt]    {$\beta $};
% Text Node
\draw (302,233.4) node [anchor=north west][inner sep=0.75pt]    {$t$};
% Text Node
\draw (229,158.4) node [anchor=north west][inner sep=0.75pt]    {$F( t)$};
% Text Node
\draw (349,158.4) node [anchor=north west][inner sep=0.75pt]    {$\rho $};
% Text Node
\draw (422,233.4) node [anchor=north west][inner sep=0.75pt]    {$\pi $};
% Text Node
\draw (418,14.4) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0,0.08,0.87}{P}$};
% Text Node
\draw (418,34.4) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.82,0.01,0.11}{Q}$};
% Text Node
\draw (104,265) node [anchor=north west][inner sep=0.75pt]   [align=left] {PR Curve \cite{sajjadi2018,simon2019revisiting}};
% Text Node
\draw (225,265) node [anchor=north west][inner sep=0.75pt]   [align=left] {Lorenz \cite{harremoes2004new, van2010renyi}};
% Text Node
\draw (348,265) node [anchor=north west][inner sep=0.75pt]   [align=left] {Div. Front. \cite{djolonga2019evaluating}};


\end{tikzpicture}



==> img/generalized_lorenz.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

% Plotting does not support converting to Tikz

% Text Node
\draw (529,172.4) node [anchor=north west][inner sep=0.75pt]    {$t$};
% Text Node
\draw (238,17.4) node [anchor=north west][inner sep=0.75pt]    {$y$};
% Text Node
\draw (302,69.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$\left(\int \phi ^{*}( f) \ dP,\int f\ dQ\right)$};
% Text Node
\draw (332,163.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 245; green, 130; blue, 49 }  ,opacity=1 ]  {$ \begin{array}{l}
t\geq \int \phi ^{*}( f) \ dP\\
y\leq \int f\ dQ
\end{array}$};


\end{tikzpicture}

==> img/gmm-pr_curve.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,205); %set diagram left start at 0, and has height of 205

%Curve Lines [id:da6936835813995819] 
\draw [draw opacity=0][fill={rgb, 255:red, 218; green, 137; blue, 147 }  ,fill opacity=1 ][line width=2.25]    (424.5,94) .. controls (432.35,95.31) and (464.5,96) .. (469.5,109) .. controls (474.5,122) and (476.83,128.78) .. (478.5,137) .. controls (480.17,145.22) and (484.17,142.59) .. (478.5,142) .. controls (472.83,141.41) and (460.53,142.08) .. (446.5,142) .. controls (432.47,141.92) and (423.93,141.31) .. (424,142) ;
%Shape: Axis 2D [id:dp41290010362368945] 
\draw  (414,142) -- (514,142)(424,52) -- (424,152) (507,137) -- (514,142) -- (507,147) (419,59) -- (424,52) -- (429,59)  ;
%Shape: Right Angle [id:dp040547899070892734] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][dash pattern={on 6.75pt off 4.5pt}][line width=2.25]  (427,69) -- (497,69) -- (497,139) ;
%Image [id:dp5560744028403637] 
\draw (226.11,90.5) node  {\includegraphics[width=222.91pt,height=78.75pt]{img/mixture-PQ.png}};
%Straight Lines [id:da6312805275784865] 
\draw [color={rgb, 255:red, 0; green, 21; blue, 223 }  ,draw opacity=1 ][line width=1.5]    (341.35,50) -- (356.03,50) ;
%Straight Lines [id:da2666403555847445] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (341.35,70) -- (356.03,70) ;

%Shape: Circle [id:dp054284216213610126] 
\draw  [draw opacity=0][fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (419.25,142) .. controls (419.25,139.38) and (421.38,137.25) .. (424,137.25) .. controls (426.62,137.25) and (428.75,139.38) .. (428.75,142) .. controls (428.75,144.62) and (426.62,146.75) .. (424,146.75) .. controls (421.38,146.75) and (419.25,144.62) .. (419.25,142) -- cycle ;
%Curve Lines [id:da054765458570643855] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (424.5,94) .. controls (432.35,95.31) and (464.5,96) .. (469.5,109) .. controls (474.5,122) and (478.5,132) .. (479.5,142) ;

% Text Node
\draw (429,40) node [anchor=north west][inner sep=0.75pt]    {$\alpha $};
% Text Node
\draw (502,115) node [anchor=north west][inner sep=0.75pt]    {$\beta $};
% Text Node
\draw (424,146.75) node [anchor=north west][inner sep=0.75pt]   [align=left] {PR Curve};
% Text Node
\draw (357.77,57) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.82,0.01,0.11}{P}\textcolor[rgb]{0.82,0.01,0.11}{_{\textcolor[rgb]{0.82,0.01,0.11}{T}}}$};
% Text Node
\draw (357.77,37) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0,0.08,0.87}{P}\textcolor[rgb]{0,0.08,0.87}{_{\textcolor[rgb]{0,0.08,0.87}{S}}}$};


\end{tikzpicture}
